BiSNN: Training Spiking Neural Networks with Binary Weights via Bayesian Learning

Artificial Neural Network (ANN)-based inference on battery-powered devices can be made more energy-efficient by restricting the synaptic weights to be binary, hence eliminating the need to perform multiplications. An alternative, emerging, approach relies on the use of Spiking Neural Networks (SNNs), biologically inspired, dynamic, event-driven models that enhance energy efficiency via the use of binary, sparse, activations. In this paper, an SNN model is introduced that combines the benefits of temporally sparse binary activations and of binary weights. Two learning rules are derived, the first based on the combination of straight-through and surrogate gradient techniques, and the second based on a Bayesian paradigm. Experiments validate the performance loss with respect to full-precision implementations, and demonstrate the advantage of the Bayesian paradigm in terms of accuracy and calibration.

==> etc.tex <==
\section{Methods}

Prior and variational distribution in minimal exponential family form:
\begin{align}
    p_{\bmw^\text{r}_0}(\bmw) &= h(\bmw) \exp\Big( (\bmw^\text{r}_0)^\top \bmphi(\bmw) - A(\bmw^\text{r}_0) \Big), \cr 
    q_{\bmw^\text{r}}(\bmw) &= h(\bmw) \exp\Big( (\bmw^\text{r})^\top \bmphi(\bmw) - A(\bmw^\text{r}) \Big)
\end{align}
In our Bernoulli distribution for binary weights $\bmw \in \{+1,-1\}^{|\bmw|}$, we have
\begin{align}
    h(\bmw) = 1,&~~~ \bmphi(\bmw) = \bmw,~~~ \bmmu = 2\bfp -1, \cr 
    \bmw^\text{r} = \frac{1}{2} \log \frac{\bfp}{1-\bfp},&~~~ A(\bmw^\text{r}) = \frac{1}{2} \log \bfp (1-\bfp).
\end{align}

Natural-gradient descent for 
\begin{align}
    \mathbb{E}_{q_{\bmw^\text{r}}(\bmw)}\Big[\set{L}_{\set{D}}(\bmw)\Big] + \rho \text{KL}\big( q_{\bmw^\text{r}}(\bmw) || p_{\bmw^\text{r}_0}(\bmw)\big).
\end{align}
In Khan's paper, for conjugate exponential family models, natural-gradients with respect to the natural parameters take a simple form: For the ratio of two terms that are conjugate to each other in the KL divergence term, the natural-gradient is equal to the difference in the natural parameter of the two terms: 
\begin{align}
    &\grad_{\bmw^\text{r}}  \mathbb{E}_{q_{\bmw^\text{r}}(\bmw)} \Big[ \log \frac{q_{\bmw^\text{r}}(\bmw)}{p_{\bmw^\text{r}_0}(\bmw)} \Big] \cr 
    &= \big[{\bf F}(\bmw^\text{r}) \big]^{-1} \grad_{\bmw^\text{r}} \mathbb{E}_{q_{\bmw^\text{r}}(\bmw)}\Big[ (\bmw^\text{r}-\bmw^\text{r}_0)^\top \bmphi(\bmw) - A(\bmw^\text{r}) \Big] \cr
    &= \bmw^\text{r} - \bmw^\text{r}_0    
\end{align}
Here, ${\bf F}$ is Fisher information matrix. Natural-gradient for the loss $\set{L}_{\set{D}}(\bmw)$ can be obtained from the gradient with respect to the mean parameters, and natural-gradient for the KL divergence can be obtained from the above equation. 
\begin{align}
    \bmw^\text{r} &\leftarrow \bmw^\text{r} - \eta \cdot \grad_{\bmw^\text{r}}\bigg( \mathbb{E}_{q_{\bmw^\text{r}}(\bmw)}\Big[\set{L}_{\set{D}}(\bmw)\Big] + \rho \text{KL}\big( q_{\bmw^\text{r}}(\bmw) || p_{\bmw^\text{r}_0}(\bmw)\big) \bigg) \cr
    &= \bmw^\text{r} - \eta \cdot \bigg(\grad_{\bmmu} \mathbb{E}_{q_{\bmw^\text{r}}(\bmw)}\Big[ \set{L}_{\set{D}}(\bmw)\Big] + \rho (\bmw^\text{r}-\bmw^\text{r}_0) \bigg) \cr 
    &= \big( 1- \eta\rho\big) \bmw^\text{r} - \eta \bigg( \grad_{\bmmu} \mathbb{E}_{q_{\bmw^\text{r}}(\bmw)}\Big[ \set{L}_{\set{D}}(\bmw)\Big] - \rho \bmw^\text{r}_0 \bigg)
\end{align}
